When Benchmarks are Targets: Revealing the Sensitivity of Large Language Model Leaderboards

Large Language Model (LLM) leaderboards based on benchmark rankings are regularly used to guide practitioners in model selection. Often, the published leaderboard rankings are taken at face value - we show this is a (potentially costly) mistake. Under existing leaderboards, the relative performance of LLMs is highly sensitive to (often minute) details. We show that for popular multiple-choice question benchmarks (e.g., MMLU), minor perturbations to the benchmark, such as changing the order of choices or the method of answer selection, result in changes in rankings up to 8 positions. We explain this phenomenon by conducting systematic experiments over three broad categories of benchmark perturbations and identifying the sources of this behavior. Our analysis results in several best-practice recommendations, including the advantage of a hybrid scoring method for answer selection. Our study highlights the dangers of relying on simple benchmark evaluations and charts the path for more robust evaluation schemes on the existing benchmarks. The code for this paper is available at https://github.com/National-Center-for-AI-Saudi-Arabia/lm-evaluation-harness.

==> figures/fixed_choice_position_pseudocode.tex <==
% \begin{algorithm}
% \caption{Experimental Design}\label{experiment}
% \begin{algorithmic}[1]

% \Procedure{RunExperiment}{}
% \For{$fs$ \textbf{in} \textbf{range}(4)}
% \For{$strat$ \textbf{in} ['fixed', 'different', 'unchanged']}
% \State Fix the position of the correct answer of every example to $fs$.
% \State Given $strat$, do the following to the test question choices after the examples:
% \If{$strat$ \textbf{is} "fixed"}
% \State Fix the position of the correct answer to $fs$
% \ElsIf{$strat$ \textbf{is} "different"}
% \State Fix the position of the correct answer to something other than $fs$
% \ElsIf{$strat$ \textbf{is} "unchanged"}
% \State Do nothing
% \EndIf
% \EndFor
% \EndFor
% \EndProcedure
% \end{algorithmic}
% \end{algorithm}

==> tables/cheatingWrong1shot.tex <==
% \begin{table}[ht]
% \centering
% \resizebox{\linewidth}{!}{
% {\color{blue}
% \begin{tabular}{lcc}
% \toprule
%                             Model &  Task acc &  $\Delta$Acc \\%Task RStd &  $\Delta$RStd \\
% \midrule
%                    \texttt{Yi-6B} &     36.13 &       -24.99  \\% 2.83 &         -0.73 \\
%          \texttt{Mistral-7B-v0.1} &     19.51 &       -40.05  \\% 4.23 &          0.10 \\
% \texttt{Mistral-7B-Instruct-v0.1} &     10.71 &       -42.77  \\% 4.79 &          0.21 \\
%            \texttt{Llama-2-7b-hf} &     24.25 &       -17.56  \\% 9.97 &          1.48 \\
%       \texttt{Llama-2-7b-chat-hf} &     16.24 &       -30.12 \\% 6.92 &         -9.18 \\
%           \texttt{Llama-2-13b-hf} &     12.76 &       -39.32 \\% 6.67 &         -5.38 \\
%      \texttt{Llama-2-13b-chat-hf} &     31.49 &       -21.63 \\% 5.81 &         -6.99 \\
%                   \texttt{Yi-34B} &     32.08 &       -41.30 \\% 4.25 &         -0.92 \\
%           \texttt{Llama-2-70b-hf} &     26.27 &       -39.17\\%  9.29 &          6.09 \\
%      \texttt{Llama-2-70b-chat-hf} &     26.26 &       -34.85 \\% 4.46 &         -6.49 \\

%                     \midrule
% $k_\tau$ = 0.422 \\
                
     
% \bottomrule
% \end{tabular}

% }
% }
% \caption{\color{blue}Evaluation of Various Large Language Models (LLMs) on the MMLU Dataset, providing incorrect answers in a One-Shot setting.}
% \label{tab:label}
% \end{table}


%                           Baseline acc  Task acc  $\Delta$Acc  Baseline RStd  Task RStd  $\Delta$RStd  Baseline acc rank  Task acc rank
% Yi-6B                           61.117    36.127      -24.990          3.568      2.833        -0.735                  3              1
% Mistral-7B-v0.1                 59.564    19.513      -40.051          4.132      4.230         0.098                  5              8
% Mistral-7B-Instruct-v0.1        53.482    10.711      -42.771          4.583      4.789         0.206                  7             11
% Llama-2-7b-hf                   41.810    24.249      -17.561          8.494      9.974         1.480                 11              7
% Llama-2-7b-chat-hf              46.368    16.244      -30.124         16.105      6.921        -9.184                 10              9
% Llama-2-13b-hf                  52.079    12.762      -39.317         12.044      6.668        -5.376                  9             10
% Llama-2-13b-chat-hf             53.119    31.491      -21.628         12.798      5.812        -6.986                  8              4
% Yi-34B                          73.380    32.082      -41.298          5.169      4.251        -0.918                  1              3
% Llama-2-70b-hf                  65.439    26.271      -39.168          3.204      9.292         6.088                  2              5
% Llama-2-70b-chat-hf             61.110    26.257      -34.853         10.945      4.458        -6.487                  4              6
% phi-2                           54.465    33.585      -20.880          4.005      2.119        -1.886                  6              2

% latex format:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[H]
\centering
\resizebox{0.7\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule
                            Model &  Task acc &  $\Delta$Acc  \\ %Task RStd &  $\Delta$RStd \\
\midrule
                   \texttt{phi-2} &     33.59 &       -20.88  \\     % 2.12 &         -1.89 \\
                   \texttt{Yi-6B} &     36.13 &       -24.99  \\    %  2.83 &         -0.73 \\
              \texttt{Mistral-7B} &     19.51 &       -40.05  \\   %    4.23 &          0.10 \\
     \texttt{Mistral-7B-Instruct} &     10.71 &       -42.77  \\    %   4.79 &          0.21 \\
              \texttt{Llama-2-7b} &     24.25 &       -17.56  \\    %   9.97 &          1.48 \\
         \texttt{Llama-2-7b-chat} &     16.24 &       -30.12  \\    %   6.92 &         -9.18 \\
             \texttt{Llama-2-13b} &     12.76 &       -39.32  \\     %  6.67 &         -5.38 \\
        \texttt{Llama-2-13b-chat} &     31.49 &       -21.63  \\    %   5.81 &         -6.99 \\
                  \texttt{Yi-34B} &     32.08 &       -41.30  \\     %  4.25 &         -0.92 \\
             \texttt{Llama-2-70b} &     26.27 &       -39.17  \\     %  9.29 &          6.09 \\
        \texttt{Llama-2-70b-chat} &     26.26 &       -34.85  \\     %  4.46 &         -6.49 \\
\midrule
$k_\tau$ = 0.382 \\
\bottomrule
\end{tabular}

}
\caption{The one-shot results on the MMLU, providing an incorrect answer in the in-context cheating experiment}
\label{tab:mmlu_cheating_wrong_1shot}
\end{table}

